Learning Riemannian Manifolds for Geodesic Motion Skills

For robots to work alongside humans and perform in unstructured environments, they must learn new motion skills and adapt them to unseen situations on the fly. This demands learning models that capture relevant motion patterns, while offering enough flexibility to adapt the encoded skills to new requirements, such as dynamic obstacle avoidance. We introduce a Riemannian manifold perspective on this problem, and propose to learn a Riemannian manifold from human demonstrations on which geodesics are natural motion skills. We realize this with a variational autoencoder (VAE) over the space of position and orientations of the robot end-effector. Geodesic motion skills let a robot plan movements from and to arbitrary points on the data manifold. They also provide a straightforward method to avoid obstacles by redefining the ambient metric in an online fashion. Moreover, geodesics naturally exploit the manifold resulting from multiple--mode tasks to design motions that were not explicitly demonstrated previously. We test our learning framework using a 7-DoF robotic manipulator, where the robot satisfactorily learns and reproduces realistic skills featuring elaborated motion patterns, avoids previously unseen obstacles, and generates novel movements in multiple-mode settings.

==> Sections/Conclusion.tex <==
We have proposed a novel LfD approach that learns a Riemannian manifold from human demonstrations and computes geodesics to recover and synthesize learned motion skills. Our approach geodesic motion generation is capable of planning movements from and to arbitrary points on the data manifold, avoiding obstacles on the fly using ambient space metric and multiple-solution trajectories. We realize this with a variational autoencoder (VAE) over the space of position and orientations of the robot end-effector. The approach is extended to graph-based geodesic computation for real-time motion generation and adaptation. Through extensive evaluation in the simulation, we show geodesic motion generation performs well in different scenarios such as grasping and pouring. 
\textbf{I REMOVED VIA POINTS FROM THE TEXT -- WE CAN DISCUSS THEM AS FUTURE WORK HERE}


